ZeRO-Offload: Democratizing Billion-Scale Model Training

Large-scale model training has been a playing ground for a limited few requiring complex model refactoring and access to prohibitively expensive GPU clusters. ZeRO-Offload changes the large model training landscape by making large model training accessible to nearly everyone. It can train models with over 13 billion parameters on a single GPU, a 10x increase in size compared to popular framework such as PyTorch, and it does so without requiring any model change from the data scientists or sacrificing computational efficiency. ZeRO-Offload enables large model training by offloading data and compute to CPU. To preserve compute efficiency, it is designed to minimize the data movement to/from GPU, and reduce CPU compute time while maximizing memory savings on GPU. As a result, ZeRO-Offload can achieve 40 TFlops/GPU on a single NVIDIA V100 GPU for 10B parameter model compared to 30TF using PyTorch alone for a 1.4B parameter model, the largest that can be trained without running out of memory. ZeRO-Offload is also designed to scale on multiple-GPUs when available, offering near linear speedup on up to 128 GPUs. Additionally, it can work together with model parallelism to train models with over 70 billion parameters on a single DGX-2 box, a 4.5x increase in model size compared to using model parallelism alone. By combining compute and memory efficiency with ease-of-use, ZeRO-Offload democratizes large-scale model training making it accessible to even data scientists with access to just a single GPU.

==> adam_eval.tex <==
{
\vspace{-10pt}
\centering
\scriptsize
\begin{tabular}{|p{1cm}|p{0.8cm}|p{0.7cm}|p{0.7cm}|}
\hline
\cellcolor[gray]{0.9} \scriptsize \textbf{\#Params}& \cellcolor[gray]{0.9} \scriptsize \textbf{CPU-Adam}& \scriptsize \cellcolor[gray]{0.9} \textbf{PT-CPU}& \scriptsize \cellcolor[gray]{0.9} \textbf{\begin{tabular}[c]{@{}l@{}}PT-GPU \\ (L2L)\end{tabular}}\\
\hline
\scriptsize 1 billion&\scriptsize 0.22&\scriptsize 1.39&\scriptsize 0.10\\
\hline
\cellcolor[gray]{0.9}\scriptsize 2 billion & \cellcolor[gray]{0.9}\scriptsize 0.51& \cellcolor[gray]{0.9}\scriptsize 2.75& \cellcolor[gray]{0.9}\scriptsize 0.26\\
\hline
\scriptsize 4 billion & \scriptsize 1.03& \scriptsize 5.71& \scriptsize 0.64\\
\hline
\cellcolor[gray]{0.9}\scriptsize 8 billion& \cellcolor[gray]{0.9}\scriptsize 2.41& \cellcolor[gray]{0.9}\scriptsize 11.93& \cellcolor[gray]{0.9}\scriptsize 0.87\\
\hline
\scriptsize 10 billion& \scriptsize 2.57& \scriptsize 14.76& \scriptsize 1.00\\
\hline
\end{tabular}
\vspace{-5pt}
\captionof{table}{Adam latency (s) for PyTorch (PT) and CPU-Adam.}
\vspace{-5pt}
\label{t:adamperf}
% \minjia{@Reza, could you please change all the digits to have 1 significant digit after the decimal? E.g., 6.381 -> 6.4.\minjia{Done.}}
}

==> related_work.tex <==
\section{Related Work}
%enable large model by partitioning
% DP, MP, ZeRO, GShard, 

\textbf{Scale out model training.}
It has been repeatedly demonstrated that deeper and larger model is critical for improving model quality in many machine learning applications.
L2L~\cite{l2l} manages memory usage in GPU layer by layer. In particular, L2L synchronously moves tensors that will be used in the upcoming layer into GPU memory for computation and keeps the rest of tensors into CPU memory for memory saving. However, different from L2L, \name leverages not only CPU memory but also CPU computation resources. By updating parameters on CPU, \name bounds communication between CPU and GPU by the number of gradients in a model, which leads to larger throughput than L2L. In addition, \name requires no model refactoring while L2L does.
%without considering the memory usages for parameters and optimizer states. 



\textbf{Scale up model training.}
Existing work scales up model size in a single node (or single GPU) through three major approaches. The first approach trades computation for memory saving by recomputing from checkpoints~\cite{chen2016training}. The second approach uses compression techniques such as using low or mixed precision~\cite{mixed_percision_training} for model training. The third approach uses an external memory such as the CPU memory as an extension of GPU memory to increase memory capacity for larger model training~\cite{vDNN_micro16,SuperNeurons_ppopp18,AutoTM_asplos20,SwapAdvisor_asplos20,Capuchin_asplos20,Layrub}. 
vDNN~\cite{vDNN_micro16} and SuperNeurons~\cite{SuperNeurons_ppopp18} focus on linear models and hence are not general. Scaling up general-propose model training on single GPU has been actively studied recently. AutoTM~\cite{AutoTM_asplos20}, SwapAdvisor~\cite{SwapAdvisor_asplos20} and Capuchin~\cite{Capuchin_asplos20} do not use any model knowledge. Instead, those efforts use a dynamic or static profiling method to decide tensor movement between GPU and CPU for memory saving. However, those efforts cannot easily scale out across devices. Also, the usability of those models is not as good as \name, because of the involvement of model change, static profiling, or offline decision making for tensor movement.
%Most of these efforts target at generic model training, whereas our solution is specifically tailored for colossal-scale models. 



